Non-convex integer programming: a deterministic solution method of the large block sale problem

We study a non-convex, nonlinear integer mathematical program with a linear constraint. This problem originates in finance and consists of selling a large predetermined quantity of a financial asset over a fixed time horizon, while maximizing the total proceeds. The selling price is modeled using a deterministic penalty function capturing the market's adverse reaction to the selling flow. From a complexity perspective, the problem is in NP. We first solve the problem exactly using dynamic programming and propose several heuristics that yield tight numerical lower bounds. We then reformulate the problem into an equivalent factorable form and derive a tight convex relaxation using McCormick inequalities. This relaxation is embedded within an adapted Branch & Bound algorithm to find the global optimum in finite time. Numerical experiments show that our methods outperform several widely used generic solvers (LocalSolver, Scip, Baron, Couenne, and Bonmin) for selected instances, but do not yield tight upper bounds, beyond small instances.

==> convbnb_verysmall_ub_f2_tab_3.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	\multicolumn{4}{|c|}{Quality - \textbf{Upper bounds}}&\multicolumn{2}{c|}{CST, $\;\;G:x\mapsto\frac{x}{1+x}$}\\
	\hline
	N&M&B\&B&\Bar&\Cou&\Sci     \\\hline
	3&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$    \\\hline
	4&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$    \\\hline
	5&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$    \\\hline
	6&$10^2$&$<\epsilon$&39.04&0.65&132.57        \\\hline
	7&$10^2$&$<\epsilon$&353.33&40.01&187.67      \\\hline
	8&$10^2$&$<\epsilon$&468.85&82.32&370.19      \\\hline
	9&$10^2$&0.19&409.88&134.94&423.27   \\\hline
	10&$10^2$&1.23&499.63&168.65&468.99  \\\hline
	\hline
	3&$10^3$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$    \\\hline
	4&$10^3$&$<\epsilon$&5.26&$<\epsilon$&$<\epsilon$           \\\hline
	5&$10^3$&$<\epsilon$&182.74&2.27&157.66       \\\hline
	6&$10^3$&0.02&511.09&48.9&283.96      \\\hline
	7&$10^3$&0.3&627.4&93.5&486.21        \\\hline
	8&$10^3$&1.01&638.12&170.31&545.56   \\\hline
	9&$10^3$&2.69&636.84&166.73&626.17   \\\hline
	10&$10^3$&10.55&642.51&207.56&629.58 \\\hline
	\hline
	3&$10^4$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$    \\\hline
	4&$10^4$&$<\epsilon$&6.69&$<\epsilon$&1.92    \\\hline
	5&$10^4$&$<\epsilon$&568.61&8.11&302.81              \\\hline
	6&$10^4$&0.09&665.92&68.73&607.2      \\\hline
	7&$10^4$&0.44&663.29&106.38&631.84     \\\hline
	8&$10^4$&1.28&655.42&169.17&655.31   \\\hline
	9&$10^4$&3.4&652.46&167.95&653.12    \\\hline
	10&$10^4$&13.58&648.3&211.86&644.87  \\\hline
\end{tabular}


==> diss_NE_GFunc_2.tex <==
Nous présentons dans cette section les fonctions de pénalité $g$ employées dans les expérimentations numériques étudions leur propriétés et discutons leur calibration.\\ 
Nous définissons les trois fonctions prototypes $G$ réelles univariées suivantes: 
\vspace{0.5cm}\\
$\begin{aligned}[t]
	G\;\left\{
	\begin{array}{l}
		x \mapsto \displaystyle \frac{x}{1+x}\\
		ou\; x\mapsto 1-\displaystyle \frac{2}{1+\sqrt{1+x}}\\
		ou\; x\mapsto \displaystyle\frac{2}{\pi}\arctan(x)\\			
	\end{array}
	\right.
\end{aligned}$
\vspace{0.5cm}\\
Les fonctions $G$ ainsi définies sont $\mathcal{C}^2$ et bornées sur $\mathbb{R}^+$. De plus, $G(0)=0\;et\;\displaystyle\lim_{+\infty}G=1$\\
Nous nous intéressons aux propriétés de convexité de $G$. 
\begin{theorem}
Les trois fonctions $G$, ainsi définies sont concaves sur $\RR+$. \\De plus,
	chacune des fonctions $x\mapsto x\cdot G(x)$ est convexe $\RR+$.
\end{theorem}
\begin{proof}
	Par calcul direct des dérivées secondes de $G$ et $x\cdot G$:\\\\
	$\begin{aligned}[t]
		G''\;\left\{
		\begin{array}{l}
			\vspace{0.2cm}
			\Big[\displaystyle\frac{x}{1+x}\Big]''=\,\frac{-2}{(1+x)^3}<0\; sur\; \RR_+\\
			\vspace{0.2cm}
			\Big[1-\displaystyle \frac{2}{1+\sqrt{1+x}}\Big]''=\frac{-(1+3\sqrt{1+x})}{2\cdot(1+x)^{3/2}\cdot(1+\sqrt{1+x})^3} < 0\; sur\; \RR_+\\
			\vspace{0.2cm}
			\Big[\displaystyle\frac{2}{\pi}\arctan(x)	\Big]''=\frac{-4\,x}{\pi(1+x)^2}\leq 0\; sur\; \RR_+\\\			
		\end{array}
		\right.
	\end{aligned}$\\\\ 
Ce qui prouve la concavité.\\\\
	$\begin{aligned}[t]
	(x\cdot G)''\;\left\{
	\begin{array}{l}
		\vspace{0.2cm}
		\Big[\displaystyle\frac{x^2}{1+x}\Big]''=\,\frac{2}{(1+x)^3}>0\; sur\; \RR_+\\
		\vspace{0.2cm}
		\Big[x-\displaystyle \frac{2\,x}{1+\sqrt{1+x}}\Big]''=\frac{4+3\,x +(x+4)\sqrt{1+x}}{2\cdot(1+x)^{3/2}\cdot(1+\sqrt{1+x})^3} > 0\; sur \; \RR_+\\
		\vspace{0.2cm}
		\Big[\displaystyle\frac{2\,x}{\pi}\arctan(x)	\Big]''=\frac{4}{\pi\big(1+x^2\big)^2}> 0\; sur\; \RR_+\\\			
	\end{array}
	\right.
\end{aligned}$\\\\
Ce qui prouve la convexité.\\
\end{proof}
Par conséquent, les prototypes associés aux fonctions de pénalité choisies sont concaves et vérifient les hypothèses du lemme \ref{lemXG} de la section \ref{sectionDPUB}, qui permet d'établir la majoration du problème \PNS\phantom{} par monotonie.\\\\
Nous définissons ensuite les fonctions de pénalités $g:x\mapsto G(\eta\, x)$, où $\eta$ est constant et dépend seulement de $G$. Soit $L$ un niveau donné , nous définissons un seuil $H$, tel que $g(L)=H$. La constante $\eta$ est donc un facteur d'échelle servant à projeter le segment $[0;L]$ (qui encadre les valeurs des variables de décisions) sur le segment $[0;H]$ (qui encadre la valeur de la pénalité sur le prix).\\\\
Les fonctions prototypes $G$ choisies sont injectives sur  $\mathbb{R}^+$, donc nous pouvons calculer leur inverse respectif $G^{-1}$, qui est donné par:
\vspace{0.5cm}\\
$\begin{aligned}[t]
	G^{-1}\;\left\{
	\begin{array}{l}
		x \mapsto \displaystyle \frac{x}{1-x}\\
		où\; x\mapsto \displaystyle \tan\big(\frac{\pi}{2}\,x\big)\\	
		où\, x\mapsto \displaystyle \frac{4\,x}{(1-x)^2}		
	\end{array}
	\right.
\end{aligned}$
\vspace{0.5cm}\\  
Nous en déduisons la valeur de $\eta=\dfrac{G^{-1}(H)}{L}$. \\\\
Nous passons aux choix des paramètres numériques $L$ et $H$.\\$L=M$ est un choix naturel car les variables de décision et leur sommes partielles sont bornées par $M$. Nous avons testé différentes valeurs pour $H \in ]0;1[$. Plus le seuil est proche de 1, plus grande est le pouvoir discriminant de la fonction de pénalité sous-jacente $g$.\\ 
Le pouvoir discriminant correspond à la distance entre une heuristique naïve comme la vente à tout prix ou la vente linéaire et l'optimum. 
Pour les expérimentations numériques, nous avons choisi $L=M$ et $H=0.99$.
La justification et le détail des tables de calibrations sont présentées à la section suivante.\\\\
Enfin, nous avons défini et calibré les fonctions de pénalité qui composent la fonction objectif de \PNS. Nous affichons les fonctions objectifs associées en dimension N=3 et M=100, avec $p$ constant, pour chaque fonction de pénalité:
\begin{figure}[H]
	\begin{center}
		\includegraphics[scale=0.75]{matlab_3_100_2.eps}
	\end{center}
	\caption{Objectif $\big(PNS_{3,100}\big)\;,\; G:x \mapsto\frac{x}{1+x}$}
\end{figure}
\newpage
\begin{figure}[H]
	\begin{center}
		\includegraphics[scale=0.75]{matlab_3_100_6.eps}
	\end{center}
	\caption{Objectif $\big(PNS_{3,100}\big)\;,\;G:x \mapsto 1-\frac{2}{1+\sqrt{1+x}}$}
\end{figure}
\begin{figure}[H]
	\begin{center}
		\includegraphics[scale=0.8]{matlab_3_100_5.eps}
	\end{center}
	\caption{Objectif $\big(PNS_{3,100}\big)\;,\;G:x \mapsto \frac{2}{\pi}\arctan(x)$}
\end{figure}\vspace{0.5cm}

\textbf{Points importants:}
\begin{itemize}
	\item Les fonctions $x\mapsto \frac{x}{1+x}$ et $x\mapsto \frac{2}{\pi}\arctan(x)$ génèrent une fonction objectif assez abrupte avec une ligne de crête assez marquée. Cela est du aux dérivées très proches des deux fonctions ($\frac{1}{(x+1)^2}$ et $\frac{1}{1+x^2}$). 
	\item L'objectif, sous la pénalité $x\mapsto 1-\frac{2}{1+\sqrt{1+x}}$, a profil beaucoup plus arrondi, et qui semble concave en dimension 3.
	\item Nous faisons bien attention à ne pas tirer de conclusions générales, à partir de la dimension 3.   
\end{itemize}


%Finally, we study the calibration process of penalty function g.\\\\ 
%\textbf{Calibration of penalty function g:}
%\begin{itemize}
%	\item We start with the selected function prototypes G: $\begin{aligned}[t]
%		\left\{
%		\begin{array}{l}
%			x \mapsto \displaystyle \frac{x}{1+x}\\
%			or\; x\mapsto 1-\displaystyle \frac{2}{1+\sqrt{1+x}}\\
%			or\; x\mapsto \displaystyle\frac{2}{\pi}\arctan(x)\\			
%		\end{array}
%		\right.
%	\end{aligned}$\\
%	\item G functions are $\mathcal{C}^2$ and bounded on $\mathbb{R}^+$. Indeed, $G(0)=0\;and\;\displaystyle\lim_{+\infty}G=1$
%	\item We then define the penalty function $g:x\mapsto G(\eta\, x)$, where $\eta$ is constant and depends only on $G$. Given a level L , we define a threshold H, such that $g(L)=H$. Hence, $\eta$ is a scaling factor aimed to transpose the positive semi-line on the $[0;L]$ segment. Selected G functions are injective on $\mathbb{R}^+$, so we can compute $\eta=\dfrac{G^{-1}(H)}{N}$, where $G^{-1}$ is given respectively by:
%	$\begin{aligned}[t]
%		\left\{
%		\begin{array}{l}
%			x \mapsto \displaystyle \frac{x}{1-x}\\
%			or\; x\mapsto \displaystyle \tan\big(\frac{\pi}{2}\,x\big)\\	
%			or\, x\mapsto \displaystyle \frac{4\,x}{(1-x)^2}		
%		\end{array}
%		\right.
%	\end{aligned}$\\   
%	\item We lastly set threshold $H$. We considered different values for $H \in ]0;1[$. The closer to 1, the more discriminatory power for g. By discriminatory, we mean the distance from naive heuristics, such as the fire sale or the uniform sale, to the optimal, is maximum. For numerical experiments, we settled for $L=N$ and $H=0.99$. Underlying justifications and calibration tables are presented in Appendix \ref{sectionCalib}.\\ 
%\end{itemize}

==> dpexact_cpu_tab1.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{CPU}&\multicolumn{2}{c|}{$\frac{x}{1+x}$}& \multicolumn{2}{c|}{$\frac{2}{\pi}\arctan(x)$}& \multicolumn{2}{c|}{$1-\frac{2}{1+\sqrt{1+x}}$}\\[2pt]
\hline
N&M&CST&AVG&CST&AVG&CST&AVG \\
\hline\hline
$10^1$&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$&$<\epsilon$             \\\hline
$10^1$&$10^3$&0.03&0.02&0.03&0.02&0.03&0.02             \\\hline
$10^1$&$10^4$&1.77&1.77&1.78&1.78&1.77&1.79             \\\hline
$10^1$&$10^5$&181&182&179&178&176&176    								 \\\hline
$10^2$&$10^3$&0.19&0.19&0.18&0.18&0.18&0.18             \\\hline
$10^2$&$10^4$&18.83&18.93&17.68&17.63&17.55&17.53       \\\hline
$10^2$&$10^5$&1829&1777&1786&1763&1752&1754             \\\hline
$10^3$&$10^5$&17 550&17 943&17 576&17 856&17 488&17 949            \\\hline
$10^1$&$10^6$&18 141&18 253&18 261&18 142&17 876&18 440            \\\hline
%$10^2$&$10^6$&178 054&179 188$^{(*)}$&180 340&NC&NC&NC     \\\hline
\end{tabular}


==> recap_avg_cpu_tab3.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{CPU}&\multicolumn{6}{c|}{AVG, $\frac{2}{\pi}arctan(x)$}\\
\hline
N&M&FS&LIS&ILS&LS&TSDP&\ub2 \\\hline
$10^1$&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&$<\epsilon$&$<\epsilon$   \\\hline
$10^1$&$10^3$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.02&$<\epsilon$          \\\hline
$10^1$&$10^4$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.11&$<\epsilon$          \\\hline
$10^1$&$10^5$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.19&$<\epsilon$          \\\hline
$10^1$&$10^6$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&2.02&$<\epsilon$          \\\hline
$10^2$&$10^3$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.15&$<\epsilon$          \\\hline
$10^2$&$10^4$&$<\epsilon$&$<\epsilon$&0.07&10&1.8&$<\epsilon$     \\\hline
$10^2$&$10^5$&$<\epsilon$&$<\epsilon$&0.14&600&6.77&$<\epsilon$  \\\hline
$10^3$&$10^5$&$<\epsilon$&$<\epsilon$&2.92&600&138.24&$<\epsilon$            \\\hline
\end{tabular}


==> recap_conv_large_f5_tab_4.tex <==
\begin{tabular}{|c|c|c|c|c||c|}
\hline
%\multicolumn{2}{|c|}{}&\multicolumn{4}{c|}{CST,$\;G: x\mapsto\frac{2}{\pi}arctan(x)$}\\[2pt] \cline{3-6}
\multicolumn{6}{|c|}{CST,$\;G: x\mapsto\frac{2}{\pi}arctan(x)$}\\[2pt] \hline
\multicolumn{2}{|c|}{Quality}&\multicolumn{3}{c||}{\textbf{Lower bounds}}&\multicolumn{1}{c|}{\textbf{Upper bounds}}\\[1pt]
\hline
N&M&Method&Best LB&\Bon&\ub2           					\\\hline
$10^1$&$10^7$&TSDP(5000)&$\times$&DNC&38.02			        \\\hline
$10^1$&$10^8$&TSDP(5000)&$\times$&DNC&38.02					\\\hline
$10^1$&$10^9$&ILS&$\times$&DNC&38.02						\\\hline
$10^2$&$10^6$&TSDP(5000)&$\times$&$<\epsilon$&364.56			\\\hline
$10^2$&$10^7$&TSDP(5000)&$\times$&$<\epsilon$&364.56			\\\hline
$10^2$&$10^8$&ILS&$<\epsilon$&$\times$&364.56		      	\\\hline
$10^2$&$10^9$&ILS&$<\epsilon$&$\times$&364.56				\\\hline
$10^3$&$10^6$&TSDP(500)&$\times$&DNC&558.72			       	\\\hline
$10^3$&$10^7$&ILS&$\times$&DNC&558.72     					\\\hline
$10^3$&$10^8$&ILS&$\times$&DNC&558.72      					\\\hline
$10^3$&$10^9$&ILS&$\times$&DNC&558.72						\\\hline
\end{tabular}

==> recap_cst_cpu_tab3.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{CPU}&\multicolumn{6}{c|}{CST, $\frac{2}{\pi}arctan(x)$}\\
\hline
N&M&FS&LIS&ILS&LS&TSDP&\ub2 \\\hline
$10^1$&$10^2$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&$<\epsilon$&$<\epsilon$   \\\hline
$10^1$&$10^3$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.02&$<\epsilon$          \\\hline
$10^1$&$10^4$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.12&$<\epsilon$          \\\hline
$10^1$&$10^5$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&0.21&$<\epsilon$           \\\hline
$10^1$&$10^6$&$<\epsilon$&$<\epsilon$&$<\epsilon$&10&2.10&$<\epsilon$            \\\hline
$10^2$&$10^3$&$<\epsilon$&$<\epsilon$&0.01&10&0.15&$<\epsilon$   \\\hline
$10^2$&$10^4$&$<\epsilon$&$<\epsilon$&0.22&10&2.12&$<\epsilon$   \\\hline
$10^2$&$10^5$&$<\epsilon$&$<\epsilon$&0.73&600&12.90&$<\epsilon$ \\\hline
$10^3$&$10^5$&$<\epsilon$&$<\epsilon$&35.42&600&213.36&$<\epsilon$           \\\hline
\end{tabular}

